Adaptive Multi-NeRF: Exploit Efficient Parallelism in Adaptive Multiple Scale Neural Radiance Field Rendering

Recent advances in Neural Radiance Fields (NeRF) have demonstrated significant potential for representing 3D scene appearances as implicit neural networks, enabling the synthesis of high-fidelity novel views. However, the lengthy training and rendering process hinders the widespread adoption of this promising technique for real-time rendering applications. To address this issue, we present an effective adaptive multi-NeRF method designed to accelerate the neural rendering process for large scenes with unbalanced workloads due to varying scene complexities. Our method adaptively subdivides scenes into axis-aligned bounding boxes using a tree hierarchy approach, assigning smaller NeRFs to different-sized subspaces based on the complexity of each scene portion. This ensures the underlying neural representation is specific to a particular part of the scene. We optimize scene subdivision by employing a guidance density grid, which balances representation capability for each Multilayer Perceptron (MLP). Consequently, samples generated by each ray can be sorted and collected for parallel inference, achieving a balanced workload suitable for small MLPs with consistent dimensions for regular and GPU-friendly computations. We aosl demonstrated an efficient NeRF sampling strategy that intrinsically adapts to increase parallelism, utilization, and reduce kernel calls, thereby achieving much higher GPU utilization and accelerating the rendering process.

==> sec/2.1_paper_sum.tex <==
\subsection{TEMP Paper Sum}

\textcolor{red}{TODO This is the TEMP paper summary session, remember to reorganize this, add actual reference and to make it into a perfect survey text as the Background/Literature section. This won't take too long time to finish}

Mip-NeRF: A Multiscale Representation for Anti-Aliasing Neural Radiance Fields

\subsubsection{Fast Neural Radiance Field Rendering}


DeRF: As there are diminishing returns in employing larger (deeper and/or wider) networks, this paper used spatially decompose a scene and dedicate smaller networks for each decomposed part to reduce rendering time. 3x faster

AutoInt: Automatic integration can be used to learn closed form solutions to the volume rendering equation. While conventional neural renderers require hundreds of samples along each ray to evaluate these integrals (and hence hundreds of costly forward passes through a network), AutoInt allows evaluating these integrals far fewer forward passes. 10x faster

DONeRF: put samples closer to surfaces in the scene. They used a depth oracle network that predicts ray sample locations for each view ray with a single network evaluation. The way to generate a prediction of surface is to use a classification network around logarithmically discretized and spherically warped depth values to encode surface locations rather than directly estimating depth. The combination of these techniques leads to DONeRF, a depth oracle network as its first step and a locally sampled shading network for ray accumulation. With DONeRF, 48x faster

KiloNeRF: use regular grid, each with very small NeRF to represent the scene. The teacher-student distillation is used for training and the speed-up did not cost much visual quality sacrificing. Smaller MLPs can definitely cost less inference time and the acceleration is significant: 2548x faster

NSVF: Instead of modeling the entire space with a single implicit function, NSVF consists of a set of voxel-bounded implicit fields organized in a sparse voxel octree. But they actually did not build very solid hierarchical structure and only utilized leaf nodes. The NSVF is progressively learned from coarse to fine with a differentiable ray-marching operation from only a set of posed 2D images of a scene. 10x faster

PlenOctree: Another very efficient cache method that tries to use spherical-harmonics cache that efficiently captures possible radiances in a hierarchical structure.

\subsection{Multiple-NeRF Methods}

In KiloNeRF, they had a very clever idea to divide the scene with regular grid, but there’s a problem: some grid might need higher resolution NeRF to represent, while some other part will be just skipped. To adaptively fit a NeRF for each grid, it’s very hard to determine the size of each cell. While if we keep the size of the grid but change the size of NeRF, it’s not regular and thus not friendly for GPU to calculate. On the other hand, we can divide the scene with bounding boxes with different sizes: like using KD-tree or Octree for the division. 

Block NeRF provided another example of using multiple-NeRF based method for a 




\subsubsection{Fast rendering}


Mip-NeRF: A Multiscale Representation for Anti-Aliasing Neural Radiance Fields
- extends NeRF to represent the scene at a continuously-valued
scale. By efficiently rendering anti-aliased conical frustums
instead of rays, mip-NeRF reduces objectionable aliasing
artifacts and significantly improves NeRF’s ability to represent
fine details, while also being 7% faster than NeRF and
half the size. Mip-NeRF (multum in parvo NeRF, as in “mipmap”), extends NeRF to simultaneously
represent the prefiltered radiance field for a continuous
space of scales.

Mip-NeRF substantially improves upon the accuracy of
NeRF, and this benefit is even greater in situations where
scene content is observed at different resolutions (i.e. setups
where the camera moves closer and farther from the
scene).

FastNeRF factorizes the NeRF volume rendering equation into two branches that are combined to give the same results as NeRF, but allow for much more efficient caching, yielding a 3000x speed up.

KiloNeRF replaces a single large NeRF-MLP with thousands of tiny MLPs, accelerating rendering by 3 orders of magnitude.

PlenOctrees introduce NeRF-SH that uses spherical harmonics to model view-dependent color, and then compresses that into a octree-like data-structure for rendering the result 3000 faster than NeRF.

SNeRG precompute and “bake” a NeRF into a new Sparse Neural Radiance Grid (SNeRG) representation, enabling real-time rendering.

RtS focuses on rendering derivatives efficiently and correctly for a variety of surface representations, including NeRF, using a fast “Surface NeRF” or sNerF renderer.

\subsubsection{Large-scale}

Block-NeRF scales NeRF to render city-scale scenes, decomposing the scene into individually trained NeRFs that are then combined to render the entire scene. Results are shown for 2.8M images. (pdf)

Mega-NeRF decomposes a large scene into cells each with a separate NeRF, allowing for reconstructions of large scenes in significantly less time than previous approaches. (pdf)

AR-NeRF: Unsupervised Learning of Depth and Defocus Effects
from Natural Images with Aperture Rendering Neural Radiance Fields

\subsubsection{Fundamental}

Mip-NeRF deals with aliasing by replacing sampling the light field by integrating over conical sections along a the viewing rays Mip-NeRF address the severe aliasing artifacts from vanilla NeRF by adapting the mip-map idea from graphics and replacing sampling the light field by integrating over conical sections along a the viewing rays.

MVSNeRF trains a model across many scenes and then renders new views conditioned on only a few posed input views, using intermediate voxelized features that encode the volume to be rendered.

DietNeRF is a very out-of-the box method that supervises the NeRF training process by a semantic loss, created by evaluating arbitrary views using CLIP, so it can learn a NeRF from a single view for arbitrary categories.

UNISURF propose to replace the density in NeRF with occupancy, and hierarchical sampling with root-finding, allowing to do both volume and surface rendering for much improved geometry.

NerfingMVS use a sparse depth map from an SfM pipeline to train a scene-specific depth network that subsequently guides the adaptive sampling strategy in NeRF.

\subsubsection{Adaptive}
NeAT: Neural Adaptive Tomography
In this paper, we present Neural Adaptive Tomography (NeAT), the first adaptive, hierarchical neural rendering pipeline for multi-view inverse rendering. Through a combination of neural features with an adaptive explicit representation, we achieve reconstruction times far superior to existing neural
inverse rendering methods. The adaptive explicit representation improves efficiency by facilitating empty space culling and concentrating samples in complex regions, while the neural features act as a neural regularized for the 3D reconstruction. 
The NeAT framework is designed specifically for the tomographic setting, which consists only of semi-transparent volumetric scenes instead of opaque objects. In this setting, NeAT outperforms the quality of existing optimization-based tomography solvers while being substantially faster.
